Unsupervised Calibration under Covariate Shift

A probabilistic model is said to be calibrated if its predicted probabilities match the corresponding empirical frequencies. Calibration is important for uncertainty quantification and decision making in safety-critical applications. While calibration of classifiers has been widely studied, we find that calibration is brittle and can be easily lost under minimal covariate shifts. Existing techniques, including domain adaptation ones, primarily focus on prediction accuracy and do not guarantee calibration neither in theory nor in practice. In this work, we formally introduce the problem of calibration under domain shift, and propose an importance sampling based approach to address it. We evaluate and discuss the efficacy of our method on both real-world datasets and synthetic datasets.

==> author.tex <==
\twocolumn[
\icmltitle{Unsupervised Calibration under Covariate Shift}

\icmlsetsymbol{equal}{*}

\begin{icmlauthorlist}
\icmlauthor{Aeiau Zzzz}{equal,to}
\icmlauthor{Bauiu C.~Yyyy}{equal,to,goo}
\icmlauthor{Cieua Vvvvv}{goo}
\icmlauthor{Iaesut Saoeu}{ed}
\icmlauthor{Fiuea Rrrr}{to}
\icmlauthor{Tateu H.~Yasehe}{ed,to,goo}
\icmlauthor{Aaoeu Iasoh}{goo}
\icmlauthor{Buiui Eueu}{ed}
\icmlauthor{Aeuia Zzzz}{ed}
\icmlauthor{Bieea C.~Yyyy}{to,goo}
\icmlauthor{Teoau Xxxx}{ed}
\icmlauthor{Eee Pppp}{ed}
\end{icmlauthorlist}

\icmlaffiliation{to}{Department of Computation, University of Torontoland, Torontoland, Canada}
\icmlaffiliation{goo}{Googol ShallowMind, New London, Michigan, USA}
\icmlaffiliation{ed}{School of Computation, University of Edenborrow, Edenborrow, United Kingdom}

\icmlcorrespondingauthor{Cieua Vvvvv}{c.vvvvv@googol.com}
\icmlcorrespondingauthor{Eee Pppp}{ep@eden.co.uk}

% You may provide any keywords that you
% find helpful for describing your paper; these are used to populate
% the "keywords" metadata in the PDF but will not be shown in the document
\icmlkeywords{Machine Learning, ICML}

\vskip 0.3in
]

% this must go after the closing bracket ] following \twocolumn[ ...

% This command actually creates the footnote in the first column
% listing the affiliations and the copyright notice.
% The command takes one argument, which is text to display at the start of the footnote.
% The \icmlEqualContribution command is standard text for equal contribution.
% Remove it (just {}) if you do not need this facility.

%\printAffiliationsAndNotice{}  % leave blank if no need to mention equal contribution
\printAffiliationsAndNotice{\icmlEqualContribution} % otherwise use the standard text.


==> commands.tex <==
%\newcommand{\stefano}[1]{{\color{red}{#1}}}
%\newcommand{\an}[1]{{\color{blue}{#1}}}

==> icmlfiles/trash.tex <==
To be concise, we hereby will denote $\gamma(x)l(h(x),y,;\beta)$ by $l_\gamma$. We use the lemma defined in \citep{cortes2010learning} (Lemma 2) to define the variance of importance weighted calibration loss in lemma. \ref{variance} as follows,
\begin{lemma} The variance of importance weighted calibration loss is bounded by the Renyi divergence $d_{\alpha}$,
\begin{eqnarray*}
    \lefteqn{Var_{\pi^{tr}}[l_\gamma] = \E_{\pi^{tr}}[(l_\gamma)^2]) - (\E_{\pi^{tr}}[l_\gamma])^2} \nonumber \\
    &   \leq d_{\alpha+1} (\pi^{te}||\pi^{tr}) (\E_{\pi^{te}}[l_\gamma)])^{1-\frac{1}{\alpha}} - (\E_{\pi^{te}}[l_\gamma))^2
\end{eqnarray*}
where Renyi divergence $d_{\alpha+1} (\pi^{te}||\pi^{tr})$ = $[\sum_x \frac{\pi^{te}(x)^{\alpha+1}}{\pi^{tr}(x)^{\alpha}} ]^{\frac{1}{\alpha}} $ where hyperparameter $\alpha > 0$.
\label{variance}
\end{lemma}
%\se{do you have a proof of this? if so, state as a lemma?}
The Renyi divergence \citep{renyi1961measures} defines the probability distribution divergence of $\pi^{te}$ from $\pi^{tr}$. From lemma. \ref{variance} it is clear that greater divergence leads to greater variance in the calibration loss estimate. \citep{you2019towards, long2018conditional} show that the distribution divergence becomes smaller after feature adaptation. While $\pi^{tr}$ and $\pi^{te}$ stay still in the input space, better adaptation model tends to show lower distribution divergence in the feature space. Let $\pi^{tr}_f$ and $\pi^{te}_f$ be the feature distributions of the train  and the test data respectively. Hence by using domain-invariant features we have $ d_{\alpha+1} (\pi^{te}_f||\pi^{tr}_f)$ smaller than $ d_{\alpha+1} (\pi^{te}||\pi^{tr}))$, thereby bounding the variance of the calibration loss estimate. Hence following \citep{you2019towards}, we step from the input space to the feature space and estimate $\gamma_f(x) = \frac{\pi^{te}_f(x)}{\pi^{tr}_f(x)}$ instead of $\gamma(x) = \frac{\pi_{te}(x)}{\pi_{tr}(x)}$. Note that these models can only reduce the distribution divergence rather than reducing it to zero. Hence we can only expect to improve over the bias created by original unweighted calibrator. Perfect calibration close to using the target labels is not guaranteed.  

\an{Further, as noted in Theorem 1 it is necessary that support of train distribution contains the support of the test distribution. When this is violated, the density ratios can grow to infinity. It is likely that the assumption is violated  in the input covariates, before aligning distributions $\pi^{tr}$ and $\pi^{te}$. After feature learning and adaptation, the features are more compact and domain-invariant. The assumption on the support of $\pi^{tr}$ in $\pi^{te}$ can hold well in the learned feature space. }


%\se{i think this is called unsupervised to supervised learning. it's a much older trick. i think it's even in the hastie-tsibhriani book} 
%\se{check hastie-tsibhriani book}

To compute density ratios we adopt an approach similar in \citep{bickel2007discriminative, you2019towards}, using Bayes' rule to derive density ratio from a model that discriminates between source (d=1) and target samples (d=0):
\begin{eqnarray}
    \lefteqn{\gamma_f(x) = \frac{\pi^{te}_f(x)}{\pi^{tr}_f(x)} = \frac{J_f(x|d=0)}{J_f(x|d=1)}} \nonumber \\
     &   = \frac{J_f(d=1)}{J_f(d=0)} \frac{J_f(d=0|x) J_f(x)}{J_f(d=1|x)J_f(x)} \\
    &   = \frac{J_f (d=1)}{J_f(d=0)} \frac{J_f (d=0|x)}{J_f(d=1|x)} \nonumber
    \label{ddre-eq-1}
\end{eqnarray}
\an{where $J_f$ is the joint distribution in the feature space . As can be seen in Eq. 3, density ratio can be decomposed into two parts - (1) $\frac{J_f (d=0|x)}{J_f(d=1|x)}$ which can be estimated by a discriminative model to distinguish source and target samples.  The model here is trained on the domain-invariant feature representation of source and target and hence follows a fully supervised learning scheme  and (2)  $\frac{J_f (d=1)}{J_f(d=0)}$ - which is a constant value that can be estimated with the sample sizes of both domains.}


\textbf{Practical considerations:}  The importance weights learnt by the discriminator may differ from the true density ratios. This can happen because, (1) the divergence between train and test is not completely zero leading to high variance (lemma. \ref{variance}) and (2) training on finite samples from source and target data leads to  over-fitting  of the discriminator on some features. This results in highly confident predictions and hence small importance weights. We follow \citep{grover2019bias} to offset these challenges using the following techniques - self-normalization, flattening, and clipping. %These techniques are not exclusive and can be combined e.g., flattened or clipped weights can be normalized.


% \begin{table*}[]
% \begin{tabular}{|c|c|c|c|c|c|c|}
% \hline
% source-target & Post-hoc model & Uncalibrated & Unweighted             & Weighted  (input layer)        & Weighted (output layer)        & Using labels \\ \hline
% A -> D   & Platt              & 0.038        & 0.184 (0.1811,0.1864)  & 0.09 (0.0866,0.0958)           & \textit{0.089 (0.0891,0.0891)} & 0.105        \\ \hline
% A -> D    & Isotonic           & 0.038        & 0.028                  & 0.032 (0.0224, 0.043)          & 0.031 (0.0311, 0.0311)         & 0.046        \\ \hline
% A -> W & Platt    & 0.038 & 0.245 & \textit{0.122}                  & 0.13           & 0.096 \\ \hline
% A -> W & Isotonic & 0.036 & 0.041 & 0.06                            & 0.041          & 0.057 \\ \hline
% D -> A   & Platt              & 0.147        & 0.285 (0.2845, 0.2848) & \textbf{0.13 (0.1219, 0.1377)} & 0.191                          & 0.134        \\ \hline
% D -> A    & Isotonic & 0.147 & 0.264 & \textit{0.259 (0.2571, 0.2627)} & 0.264          & 0.036 \\ \hline
% D -> W   & Platt    & 0.158 & 0.091 & \textbf{0.03 (0.0249, 0.0363)}  & 0.043          & 0.013 \\ \hline
% D -> W   & Isotonic & 0.158 & 0.036 & \textbf{0.02 (0.0163, 0.028)}   & 0.036          & 0.027 \\ \hline
% W -> A & Platt    & 0.045 & 0.265 & \textit{0.14}                   & 0.181          & 0.147 \\ \hline
% W -> A & Isotonic & 0.045 & 0.232 & 0.251                           & 0.232          & 0.042 \\ \hline
% W -> D  & Platt    & 0.096 & 0.024 & 0.019 (0.0176, 0.0214)          & \textbf{0.018} & 0.013 \\ \hline
% W -> D   & Isotonic & 0.096 & 0.014 & \textbf{0.012}                  & 0.014          & 0.02  \\ \hline
% \end{tabular}
% \caption{ECE score of the baselines and the proposed method on Office-31 dataset. The model calibrated is Resnet-50 pretrained model trained on the source dataset and tested on the target dataset. }
% \label{tab:office_3}
% \end{table*}


\begin{table*}
  \floatsetup{capposition=bottom, floatrowsep=qquad,captionskip=2pt}
  \begin{floatrow}[2]
    \makegapedcells
    \ttabbox%
     {\setlength\tabcolsep{4pt}
\begin{tabularx}{0.55\textwidth}{@{} l l l l l l l @{}}
\toprule
Method&A$\rightarrow$D&A$\rightarrow$W&D$\rightarrow$A&D$\rightarrow$W&W$\rightarrow$A&W$\rightarrow$D\\
\midrule
Uncalibrated & 0.038 & 0.036 & 0.147 & 0.158 & 0.045 & 0.096 \\ \hline
Unweighted   & 0.082 & 0.06  & 0.278 & 0.093 & 0.199 & 0.085 \\
Weighted & 0.125 & \textit{0.051} & \textbf{0.06} & \textbf{0.041} & \textit{0.052} & \textbf{0.083} \\
Using target & 0.105 & 0.062 & 0.057 & 0.06  & 0.026 & 0.013 \\ \hline \hline
Wnweighted   & 0.040 & 0.045 & 0.145          & 0.028 & 0.136                   & 0.023         \\
Weighted     & 0.047 & 0.081 & \textbf{0.134} & 0.031 & \textit{\textbf{0.039}} & \textbf{0.02} \\
Using target  & 0.047 & 0.030 & 0.031          & 0.029 & 0.028                   & 0.013        \\
\bottomrule
\end{tabularx}{\caption{ECE scores of Platt scaling (top) and t-scaling (bottom), comparing  the baselines and the proposed method on Office-31 dataset. Importance weight are obtained from discriminative density ratio estimation.}
      \label{tab:office_31}}}
    \hfill%
    \ttabbox%
   {\setlength\tabcolsep{3pt}
\begin{tabularx}{0.3\textwidth}{@{} l l l @{}}
\toprule
Method&U$\rightarrow$M&M$\rightarrow$U\\
\midrule
uncalibrated & 0.309          & 0.206          \\ \hline
unweighted   & 0.134          & 0.258          \\
weightes     & \textbf{0.132} & \textbf{0.077} \\
using target & 0.035          & 0.023    \\ \hline \hline
unweighted   & 0.154          & 0.196         \\
weighted     & \textbf{0.108} & \textbf{0.13} \\
using target & 0.140           & 0.042 \\
\bottomrule
\end{tabularx}}
   {\caption{ECE scores of Platt scaling (top) and t-scaling (bottom), comparing  the baselines and the proposed method on digits dataset. Importance weight are obtained from discriminative density ratio estimation} \label{tab: digits}}
  \end{floatrow}
\end{table*}


\begin{table*}[t]
\begin{center}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
source-target & Post-hoc & Uncalibrated & Unweighted & Weighted (in layer) & Weighted (out layer) & \begin{tabular}[c]{@{}c@{}} Using target \end{tabular} \\ \hline
M $\rightarrow$ U & Platt  &  0.206 & 0.359  & 0.122  & \textbf{0.118} & 0.008  \\ \hline
M $\rightarrow$ U  & Isotonic  &  0.206 & 0.112  & \textbf{0.103}  &  \textbf{0.103} & 0.05\\ \hline
U $\rightarrow$ M & Platt  &  0.308 & 0.391  & \textit{0.364}  & 0.368 & 0.036  \\ \hline
U $\rightarrow$ M & Isotonic & 0.308  &  0.141 &  \textbf{0.138} & 0.141  &  0.028 \\ \hline
S $\rightarrow$ M & Platt &  &  &  &  &  \\ \hline
S $\rightarrow$ M &  Isotonic &  &  &  &  &  \\ \hline
\end{tabular}
\caption{ECE score of the baselines and the proposed method on digits dataset. The model being calibrated is CDAN (cite)- domain adaptated on source and target. In \textbf{bold} we highlight weighted calibration outperforming the uncalibrated ECE. In \textit{italics} we highlight weighted calibration which reduces the bias in unweighted calibration but still performs worse than uncalibrated ECE.}
\label{tab:my-table}
\end{center}
\end{table*}

\begin{table*}[t]
\begin{center}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
source-target & Post-hoc & Uncalibrated & Unweighted             & Weighted (in layer)        & Weighted (out layer)        & Using target \\ \hline
A $\rightarrow$ D   & Platt              & 0.038        & 0.184   & 0.09         & \textit{0.089} & 0.105        \\ \hline
A  $\rightarrow$ D    & Isotonic           & 0.038        & 0.028                  & 0.032          & 0.031       & 0.046        \\ \hline
A  $\rightarrow$ W & Platt    & 0.038 & 0.245 & \textit{0.122}                  & 0.13           & 0.096 \\ \hline
A  $\rightarrow$ W & Isotonic & 0.036 & 0.041 & 0.06                            & 0.041          & 0.057 \\ \hline
D  $\rightarrow$ A   & Platt              & 0.147        & 0.285 & \textbf{0.13} & 0.191                          & 0.134        \\ \hline
D  $\rightarrow$ A    & Isotonic & 0.147 & 0.264 & \textit{0.259} & 0.264          & 0.036 \\ \hline
D  $\rightarrow$ W   & Platt    & 0.158 & 0.091 & \textbf{0.03}  & 0.043          & 0.013 \\ \hline
D  $\rightarrow$ W   & Isotonic & 0.158 & 0.036 & \textbf{0.02}   & 0.036          & 0.027 \\ \hline
W  $\rightarrow$ A & Platt    & 0.045 & 0.265 & \textit{0.14}                   & 0.181          & 0.147 \\ \hline
W  $\rightarrow$ A & Isotonic & 0.045 & 0.232 & 0.251                           & 0.232          & 0.042 \\ \hline
W  $\rightarrow$ D  & Platt    & 0.096 & 0.024 & 0.019          & \textbf{0.018} & 0.013 \\ \hline
W  $\rightarrow$ D   & Isotonic & 0.096 & 0.014 & \textbf{0.012}                  & 0.014          & 0.02  \\ \hline
\end{tabular}
\caption{ECE score of the baselines and the proposed method on Office-31 dataset. The model being calibrated is pretrained Resnet-50 trained on the source and tested on the target. In \textbf{bold} we highlight weighted calibration outperforming the uncalibrated ECE. In \textit{italics} we highlight weighted calibration which reduces the bias in unweighted calibration but still performs worse than uncalibrated ECE. }
\label{tab:office_3}
\end{center}
\end{table*}

\begin{table*}[t]
\begin{center}
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
\begin{tabular}[c]{@{}c@{}}CIFAR-10\\ classes\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Post-hoc\\ method\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Mixing ratio\\ source\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Mixing ratio\\ target\end{tabular} &
  Uncalibrated &
  Unweighted &
  GT Weighted &
 
  \begin{tabular}[c]{@{}c@{}}Using target\end{tabular} \\ \hline
2\&7 & Platt    & 1:4 & 4:1 &  0.103 (0.061)   &   0.126 (0.045) & \textbf{0.039 (0.009) } &   0.033 (0.007)  \\ \hline
%2\&7 & Isotonic & 1:4 & 4:1 & 0.089 (0.027) &   0.18 (0.023)     & \textbf{0.017 (0.004)} & 0.013 (0.004) \\ \hline
2\&7 & T-scaling & 1:4 & 4:1 & 0.111 (0.032) & 0.104 (0.023)       & \textbf{0.032 (0.007)} &  0.023 (0.009) \\ \hline
1\&8 & Platt    & 2:5 & 3:4 &  0.011 (0.006)  & 0.027 (0.007) &  0.027 (0.006)  & 0.026 (0.003)  \\ \hline
%1\&8 & Isotonic & 2:5 & 3:4 & 0.017 (0.014) & 0.019 (0.006)   &   \textbf{0.004 (0.001)} &   0.007 (0.002) \\ \hline
1\&8 & T-scaling & 2:5 & 3:4 & 0.01 (0.004)  & 0.006 (0.002)    &   0.009 (0.003) &  0.007 (0.002) \\ \hline
3\&4 & Platt    & 5:1 & 1:3 & 0.157 (0.055) & 0.184 (0.036)  & \textbf{0.044 (0.009)} & 0.036 (0.007) \\ \hline
%3\&4 & Isotonic & 5:1 & 1:3 & 0.145 (0.072) & 0.243 (0.041)  &  \textbf{0.023 (0.006)} &  0.02 (0.004) \\ \hline
3\&4 & T-scaling & 5:1 & 1:3 & 0.177 (0.049) & 0.164 (0.039) & \textbf{0.038 (0.009)}  &  0.034 (0.009) \\ \hline
6\&9 & Platt    & 2:3 & 5:1 & 0.013 (0.006)  & 0.029 (0.011) & \textit{0.018 (0.008)} &  0.018 (0.007) \\ \hline
%6\&9 & Isotonic & 2:3 & 5:1 &  0.01 (0.004)   & 0.05 (0.012) & \textbf{0.007 (0.003)} & 0.009 (0.003) \\ \hline
6\&9 & T-scaling & 2:3 & 5:1 &  0.012 (0.005) & 0.011 (0.006)  & \textbf{0.009 (0.004)} & 0.007 (0.001) \\ \hline
\end{tabular}
\caption{ECE scores of the baselines and the proposed method on pseudo-synthetic datasets. The model being calibrated is LeNet-5 trained on subclasses of CIFAR-10 present in different mixing ratios in source and target. The weighted method here uses ground truth density ratios for calibration. In \textbf{bold} we highlight weighted calibration outperforming the uncalibrated ECE.  In \textit{italics} we highlight weighted calibration which reduces the bias in unweighted calibration but still performs worse than uncalibrated ECE. Brackets show the standard deviation across 10 different train-test splits.}
\label{tab:syn}
\end{center}
\end{table*}

 \begin{table}
\setlength\tabcolsep{1.5pt}
\begin{tabularx}{\textwidth}{@{} l l l l l  @{}}
\toprule
Method & S1 \rightarrow T1 & S2 \rightarrow T2 & S3 \rightarrow T3 & S4 \rightarrow T4 & \\ 
\midrule
Uncalibrated & 0.13 (0.09) &  0.01 (0.01) &  0.14 (0.05) & 0.02 (0.02) \\
Unweighted & 0.124 (0.060) & 0.007 (0.003) &  0.144 (0.043) & 0.013 (0.008) \\
Weighted &  0.030 (0.018)& 0.005 (0.001) & 0.03 (0.011) & 0.007 (0.001)  \\
Using label &  0.027 (0.018) & 0.005 (0.001) &  0.029 (0.011) & 0.007 (0.003) \\

\bottomrule
\end{tabularx}
\caption{Office-home dataset trained using CDAN. }
\label{tb:Table 2}
\end{table}



%We use the CIFAR-10 classification dataset which consists of 60K color images distributed equally across ten object classes \citep{krizhevsky2009learning}. We randomly pick two classes and use them to define a binary classification task. In order to create a dataset shift, we consider the classes with different ratios for the source and target domain shown in Table \ref{tab:syn} as ($S_i \rightarrow T_i$). For example, if the source consists of $1:4$ ratio of class 1 and class 2 than the target with ratio of $4:1$ for the classes can be seen to have a dataset shift. To create ratio values greater than one, we duplicate the data points of the class. Finding the ground truth importance weights from the mixing ratios of source and target data is straightforward. In the given example, the source points from class 1 have an importance weight of 4 and the source points in class 2 have an importance weight of 0.25 for the given target. Using these ground truth importance weights we do a weighted calibration of a LeNet-5 classifier  trained on the labeled source data.  We use 70\% of the source data for training the classifier and 30\%  as validation data for calibration. For testing, we use 30\% of the target data to compute the ECE. We consider 10 different train, validation and test splits and report the mean in Table \ref{tab:syn}. (standard deviation in supplementary). We note that the weighted calibration significantly outperforms unweighted and uncalibrated models except in $S_2 \rightarrow T_2$ where the source ratio is close to the target ratio and hence the std error bars overlap.  

%In Table \ref{tab:syn}, we compare the calibration performance of our method  with the baselines. We see that the unweighted source calibrator has a large performance gap compared to the target-calibrated method. Infact in some cases we see that an unweighted calibrator trained on the source data can perform worse than an uncalibrated model on the target data. Our weighted calibrator reduces this gap and performs as well as the target-calibrated (lower bound) but by using only the labeled source data.

%We compare the performance of our calibration method (Weighted) to three baselines: (1) Uncalibrated, here we consider the original models prediction probabilities without any post-hoc calibration (2) unweighted, here the post-hoc calibrator is trained on the source domain which treats both the source and the target domains as if they came from the same distribution (3) target-calibrated, here the post-hoc calibrator is trained on the labeled target domain. This can be considered as a empirical lower-bound on the calibration performance for the target data. 

%In this section, we evaluate the efficacy of the importance weighting technique to adapt two post-hoc calibration methods, platt scaling and temperature scaling (t-scaling), to domain shift. We use the Expected Calibration Error or ECE (bins fixed to 10) discussed in Sec. \ref{rwork} to measure the calibration performance on the target data. We consider experiments on both pseudo-real and real world datasets: (1) For the pseudo-real world datasets in Sec. \ref{prdataset} we created a source and a target domain with an artificial sample selection bias. This allows us to compute the ground truth density ratios which we directly use for importance weighting. We train a classifier using only the source data and   perform a simulated study to understand the different parameters that effect the calibration of the classifier under domain shift.  (2) On real world domain shifted datasets in Sec. \ref{real-data} we derive the importance weights using the discriminative density ratio estimation method (Sec. \ref{ddre}) to use them for weighted calibration. The classifiers used here include both ImageNet pre-trained ResNet50 \citep{he2016deep} models trained only on the labeled source data and popular domain adapted models such as CDAN \citep{long2018conditional} which use both labeled source data and unlabeled target data.

% and DANN \cite{ganin2016domain}
%train/validation spli

%In this section, we evaluate calibration performance on real world datasets using classifiers trained only on source (using pre-trained ResNet50) and a range of domain adapted classifiers (LeNet-5 and ResNet50 trained using CDAN\footnote{We train using codes provided by authors}, pre-trained ResNet-50). The accuracy of all the models is reported in the supplementary. We divide both source and target data into 70/30 splits (we directly use standard train/test is available). For the source, the larger split is used for training and the smaller split is used as validation for the post-hoc calibration method. For the target, the larger split is used for testing  and the smaller split is used to train the target-calibrated model. To obtain importance weights for out method we train a discriminator (2-hidden layer MLP) on domain invariant features as discussed in Sec.\ref{ddre}. We do normalization on the obtained weights, and leave experimentation with flattening and clipping for future work. We experiment with different discriminator and calibrator initializations keeping the classifier and dataset fixed and report the mean performance (standard deviation in supplementary).  

==> old.tex <==
\subsection{Submitting Papers}

\textbf{Paper Deadline:} The deadline for paper submission that is
advertised on the conference website is strict. If your full,
anonymized, submission does not reach us on time, it will not be
considered for publication. 

\textbf{Anonymous Submission:} ICML uses double-blind review: no identifying
author information may appear on the title page or in the paper
itself. Section~\ref{author info} gives further details.

\textbf{Simultaneous Submission:} ICML will not accept any paper which,
at the time of submission, is under review for another conference or
has already been published. This policy also applies to papers that
overlap substantially in technical content with conference papers
under review or previously published. ICML submissions must not be
submitted to other conferences during ICML's review period. Authors
may submit to ICML substantially different versions of journal papers
that are currently under review by the journal, but not yet accepted
at the time of submission. Informal publications, such as technical
reports or papers in workshop proceedings which do not appear in
print, do not fall under these restrictions.

\medskip

Authors must provide their manuscripts in \textbf{PDF} format.
Furthermore, please make sure that files contain only embedded Type-1 fonts
(e.g.,~using the program \texttt{pdffonts} in linux or using
File/DocumentProperties/Fonts in Acrobat). Other fonts (like Type-3)
might come from graphics files imported into the document.

Authors using \textbf{Word} must convert their document to PDF\@. Most
of the latest versions of Word have the facility to do this
automatically. Submissions will not be accepted in Word format or any
format other than PDF\@. Really. We're not joking. Don't send Word.

Those who use \textbf{\LaTeX} should avoid including Type-3 fonts.
Those using \texttt{latex} and \texttt{dvips} may need the following
two commands:

{\footnotesize
\begin{verbatim}
dvips -Ppdf -tletter -G0 -o paper.ps paper.dvi
ps2pdf paper.ps
\end{verbatim}}
It is a zero following the ``-G'', which tells dvips to use
the config.pdf file. Newer \TeX\ distributions don't always need this
option.

Using \texttt{pdflatex} rather than \texttt{latex}, often gives better
results. This program avoids the Type-3 font problem, and supports more
advanced features in the \texttt{microtype} package.

\textbf{Graphics files} should be a reasonable size, and included from
an appropriate format. Use vector formats (.eps/.pdf) for plots,
lossless bitmap formats (.png) for raster graphics with sharp lines, and
jpeg for photo-like images.

The style file uses the \texttt{hyperref} package to make clickable
links in documents. If this causes problems for you, add
\texttt{nohyperref} as one of the options to the \texttt{icml2019}
usepackage statement.


\subsection{Submitting Final Camera-Ready Copy}

The final versions of papers accepted for publication should follow the
same format and naming convention as initial submissions, except that
author information (names and affiliations) should be given. See
Section~\ref{final author} for formatting instructions.

The footnote, ``Preliminary work. Under review by the International
Conference on Machine Learning (ICML). Do not distribute.'' must be
modified to ``\textit{Proceedings of the
$\mathit{36}^{th}$ International Conference on Machine Learning},
Long Beach, USA, 2019.
Copyright 2019 by the author(s).''

For those using the \textbf{\LaTeX} style file, this change (and others) is
handled automatically by simply changing
$\mathtt{\backslash usepackage\{icml2019\}}$ to
$$\mathtt{\backslash usepackage[accepted]\{icml2019\}}$$
Authors using \textbf{Word} must edit the
footnote on the first page of the document themselves.

Camera-ready copies should have the title of the paper as running head
on each page except the first one. The running title consists of a
single line centered above a horizontal rule which is $1$~point thick.
The running head should be centered, bold and in $9$~point type. The
rule should be $10$~points above the main text. For those using the
\textbf{\LaTeX} style file, the original title is automatically set as running
head using the \texttt{fancyhdr} package which is included in the ICML
2019 style file package. In case that the original title exceeds the
size restrictions, a shorter form can be supplied by using

\verb|\icmltitlerunning{...}|

just before $\mathtt{\backslash begin\{document\}}$.
Authors using \textbf{Word} must edit the header of the document themselves.

\section{Format of the Paper}

All submissions must follow the specified format.

\subsection{Length and Dimensions}

Submitted papers can be up to eight pages long, not including references, and up to twelve pages when references and acknowledgments are included.
Acknowledgements should be limited to grants and people who contributed to the paper.
Any submission that exceeds
this page limit, or that diverges significantly from the specified format,
will be rejected without review.

The text of the paper should be formatted in two columns, with an
overall width of 6.75~inches, height of 9.0~inches, and 0.25~inches
between the columns. The left margin should be 0.75~inches and the top
margin 1.0~inch (2.54~cm). The right and bottom margins will depend on
whether you print on US letter or A4 paper, but all final versions
must be produced for US letter size.

The paper body should be set in 10~point type with a vertical spacing
of 11~points. Please use Times typeface throughout the text.

\subsection{Title}

The paper title should be set in 14~point bold type and centered
between two horizontal rules that are 1~point thick, with 1.0~inch
between the top rule and the top edge of the page. Capitalize the
first letter of content words and put the rest of the title in lower
case.

\subsection{Author Information for Submission}
\label{author info}

ICML uses double-blind review, so author information must not appear. If
you are using \LaTeX\/ and the \texttt{icml2019.sty} file, use
\verb+\icmlauthor{...}+ to specify authors and \verb+\icmlaffiliation{...}+ to specify affiliations. (Read the TeX code used to produce this document for an example usage.) The author information
will not be printed unless \texttt{accepted} is passed as an argument to the
style file.
Submissions that include the author information will not
be reviewed.

\subsubsection{Self-Citations}

If you are citing published papers for which you are an author, refer
to yourself in the third person. In particular, do not use phrases
that reveal your identity (e.g., ``in previous work \cite{langley00}, we
have shown \ldots'').

Do not anonymize citations in the reference section. The only exception are manuscripts that are
not yet published (e.g., under submission). If you choose to refer to
such unpublished manuscripts \cite{anonymous}, anonymized copies have
to be submitted
as Supplementary Material via CMT\@. However, keep in mind that an ICML
paper should be self contained and should contain sufficient detail
for the reviewers to evaluate the work. In particular, reviewers are
not required to look at the Supplementary Material when writing their
review.

\subsubsection{Camera-Ready Author Information}
\label{final author}

If a paper is accepted, a final camera-ready copy must be prepared.
%
For camera-ready papers, author information should start 0.3~inches below the
bottom rule surrounding the title. The authors' names should appear in 10~point
bold type, in a row, separated by white space, and centered. Author names should
not be broken across lines. Unbolded superscripted numbers, starting 1, should
be used to refer to affiliations.

Affiliations should be numbered in the order of appearance. A single footnote
block of text should be used to list all the affiliations. (Academic
affiliations should list Department, University, City, State/Region, Country.
Similarly for industrial affiliations.)

Each distinct affiliations should be listed once. If an author has multiple
affiliations, multiple superscripts should be placed after the name, separated
by thin spaces. If the authors would like to highlight equal contribution by
multiple first authors, those authors should have an asterisk placed after their
name in superscript, and the term ``\textsuperscript{*}Equal contribution"
should be placed in the footnote block ahead of the list of affiliations. A
list of corresponding authors and their emails (in the format Full Name
\textless{}email@domain.com\textgreater{}) can follow the list of affiliations.
Ideally only one or two names should be listed.

A sample file with author names is included in the ICML2019 style file
package. Turn on the \texttt{[accepted]} option to the stylefile to
see the names rendered. All of the guidelines above are implemented
by the \LaTeX\ style file.

\subsection{Abstract}

The paper abstract should begin in the left column, 0.4~inches below the final
address. The heading `Abstract' should be centered, bold, and in 11~point type.
The abstract body should use 10~point type, with a vertical spacing of
11~points, and should be indented 0.25~inches more than normal on left-hand and
right-hand margins. Insert 0.4~inches of blank space after the body. Keep your
abstract brief and self-contained, limiting it to one paragraph and roughly 4--6
sentences. Gross violations will require correction at the camera-ready phase.

\subsection{Partitioning the Text}

You should organize your paper into sections and paragraphs to help
readers place a structure on the material and understand its
contributions.

\subsubsection{Sections and Subsections}

Section headings should be numbered, flush left, and set in 11~pt bold
type with the content words capitalized. Leave 0.25~inches of space
before the heading and 0.15~inches after the heading.

Similarly, subsection headings should be numbered, flush left, and set
in 10~pt bold type with the content words capitalized. Leave
0.2~inches of space before the heading and 0.13~inches afterward.

Finally, subsubsection headings should be numbered, flush left, and
set in 10~pt small caps with the content words capitalized. Leave
0.18~inches of space before the heading and 0.1~inches after the
heading.

Please use no more than three levels of headings.

\subsubsection{Paragraphs and Footnotes}

Within each section or subsection, you should further partition the
paper into paragraphs. Do not indent the first line of a given
paragraph, but insert a blank line between succeeding ones.

You can use footnotes\footnote{Footnotes
should be complete sentences.} to provide readers with additional
information about a topic without interrupting the flow of the paper.
Indicate footnotes with a number in the text where the point is most
relevant. Place the footnote in 9~point type at the bottom of the
column in which it appears. Precede the first footnote in a column
with a horizontal rule of 0.8~inches.\footnote{Multiple footnotes can
appear in each column, in the same order as they appear in the text,
but spread them across columns and pages if possible.}

\begin{figure}[ht]
\vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=\columnwidth]{icml_numpapers}}
\caption{Historical locations and number of accepted papers for International
Machine Learning Conferences (ICML 1993 -- ICML 2008) and International
Workshops on Machine Learning (ML 1988 -- ML 1992). At the time this figure was
produced, the number of accepted papers for ICML 2008 was unknown and instead
estimated.}
\label{icml-historical}
\end{center}
\vskip -0.2in
\end{figure}

\subsection{Figures}

You may want to include figures in the paper to illustrate
your approach and results. Such artwork should be centered,
legible, and separated from the text. Lines should be dark and at
least 0.5~points thick for purposes of reproduction, and text should
not appear on a gray background.

Label all distinct components of each figure. If the figure takes the
form of a graph, then give a name for each axis and include a legend
that briefly describes each curve. Do not include a title inside the
figure; instead, the caption should serve this function.

Number figures sequentially, placing the figure number and caption
\emph{after} the graphics, with at least 0.1~inches of space before
the caption and 0.1~inches after it, as in
Figure~\ref{icml-historical}. The figure caption should be set in
9~point type and centered unless it runs two or more lines, in which
case it should be flush left. You may float figures to the top or
bottom of a column, and you may set wide figures across both columns
(use the environment \texttt{figure*} in \LaTeX). Always place
two-column figures at the top or bottom of the page.

\subsection{Algorithms}

If you are using \LaTeX, please use the ``algorithm'' and ``algorithmic''
environments to format pseudocode. These require
the corresponding stylefiles, algorithm.sty and
algorithmic.sty, which are supplied with this package.
Algorithm~\ref{alg:example} shows an example.

\begin{algorithm}[tb]
   \caption{Bubble Sort}
   \label{alg:example}
\begin{algorithmic}
   \STATE {\bfseries Input:} data $x_i$, size $m$
   \REPEAT
   \STATE Initialize $noChange = true$.
   \FOR{$i=1$ {\bfseries to} $m-1$}
   \IF{$x_i > x_{i+1}$}
   \STATE Swap $x_i$ and $x_{i+1}$
   \STATE $noChange = false$
   \ENDIF
   \ENDFOR
   \UNTIL{$noChange$ is $true$}
\end{algorithmic}
\end{algorithm}

\subsection{Tables}

You may also want to include tables that summarize material. Like
figures, these should be centered, legible, and numbered consecutively.
However, place the title \emph{above} the table with at least
0.1~inches of space before the title and the same after it, as in
Table~\ref{sample-table}. The table title should be set in 9~point
type and centered unless it runs two or more lines, in which case it
should be flush left.

% Note use of \abovespace and \belowspace to get reasonable spacing
% above and below tabular lines.

\begin{table}[t]
\caption{Classification accuracies for naive Bayes and flexible
Bayes on various data sets.}
\label{sample-table}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcccr}
\toprule
Data set & Naive & Flexible & Better? \\
\midrule
Breast    & 95.9$\pm$ 0.2& 96.7$\pm$ 0.2& $\surd$ \\
Cleveland & 83.3$\pm$ 0.6& 80.0$\pm$ 0.6& $\times$\\
Glass2    & 61.9$\pm$ 1.4& 83.8$\pm$ 0.7& $\surd$ \\
Credit    & 74.8$\pm$ 0.5& 78.3$\pm$ 0.6&         \\
Horse     & 73.3$\pm$ 0.9& 69.7$\pm$ 1.0& $\times$\\
Meta      & 67.1$\pm$ 0.6& 76.5$\pm$ 0.5& $\surd$ \\
Pima      & 75.1$\pm$ 0.6& 73.9$\pm$ 0.5&         \\
Vehicle   & 44.9$\pm$ 0.6& 61.5$\pm$ 0.4& $\surd$ \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

Tables contain textual material, whereas figures contain graphical material.
Specify the contents of each row and column in the table's topmost
row. Again, you may float tables to a column's top or bottom, and set
wide tables across both columns. Place two-column tables at the
top or bottom of the page.

\subsection{Citations and References}

Please use APA reference format regardless of your formatter
or word processor. If you rely on the \LaTeX\/ bibliographic
facility, use \texttt{natbib.sty} and \texttt{icml2019.bst}
included in the style-file package to obtain this format.

Citations within the text should include the authors' last names and
year. If the authors' names are included in the sentence, place only
the year in parentheses, for example when referencing Arthur Samuel's
pioneering work \yrcite{Samuel59}. Otherwise place the entire
reference in parentheses with the authors and year separated by a
comma \cite{Samuel59}. List multiple references separated by
semicolons \cite{kearns89,Samuel59,mitchell80}. Use the `et~al.'
construct only for citations with three or more authors or after
listing all authors to a publication in an earlier reference \cite{MachineLearningI}.

Authors should cite their own work in the third person
in the initial version of their paper submitted for blind review.
Please refer to Section~\ref{author info} for detailed instructions on how to
cite your own papers.

Use an unnumbered first-level section heading for the references, and use a
hanging indent style, with the first line of the reference flush against the
left margin and subsequent lines indented by 10 points. The references at the
end of this document give examples for journal articles \cite{Samuel59},
conference publications \cite{langley00}, book chapters \cite{Newell81}, books
\cite{DudaHart2nd}, edited volumes \cite{MachineLearningI}, technical reports
\cite{mitchell80}, and dissertations \cite{kearns89}.

Alphabetize references by the surnames of the first authors, with
single author entries preceding multiple author entries. Order
references for the same authors by year of publication, with the
earliest first. Make sure that each reference includes all relevant
information (e.g., page numbers).

Please put some effort into making references complete, presentable, and
consistent. If using bibtex, please protect capital letters of names and
abbreviations in titles, for example, use \{B\}ayesian or \{L\}ipschitz
in your .bib file.

\subsection{Software and Data}

We strongly encourage the publication of software and data with the
camera-ready version of the paper whenever appropriate. This can be
done by including a URL in the camera-ready copy. However, do not
include URLs that reveal your institution or identity in your
submission for review. Instead, provide an anonymous URL or upload
the material as ``Supplementary Material'' into the CMT reviewing
system. Note that reviewers are not required to look at this material
when writing their review.

% Acknowledgements should only appear in the accepted version.
\section*{Acknowledgements}

\textbf{Do not} include acknowledgements in the initial version of
the paper submitted for blind review.

If a paper is accepted, the final camera-ready version can (and
probably should) include acknowledgements. In this case, please
place such acknowledgements in an unnumbered section at the
end of the paper. Typically, this will include thanks to reviewers
who gave useful comments, to colleagues who contributed to the ideas,
and to funding agencies and corporate sponsors that provided financial
support.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% DELETE THIS PART. DO NOT PLACE CONTENT AFTER THE REFERENCES!
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\appendix
\section{Do \emph{not} have an appendix here}

\textbf{\emph{Do not put content after the references.}}
%
Put anything that you might normally include after the references in a separate
supplementary file.

We recommend that you build supplementary material in a separate document.
If you must create one PDF and cut it up, please be careful to use a tool that
doesn't alter the margins, and that doesn't aggressively rewrite the PDF file.
pdftk usually works fine. 

\textbf{Please do not use Apple's preview to cut off supplementary material.} In
previous years it has altered margins, and created headaches at the camera-ready
stage. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
